Black Boxes and Looking Glasses: Multilevel Symmetries, Reflection Planes, and Convex Optimization in Deep Networks

We show that training deep neural networks (DNNs) with absolute value activation and arbitrary input dimension can be formulated as equivalent convex Lasso problems with novel features expressed using geometric algebra. This formulation reveals geometric structures encoding symmetry in neural networks. Using the equivalent Lasso form of DNNs, we formally prove a fundamental distinction between deep and shallow networks: deep networks inherently favor symmetric structures in their fitted functions, with greater depth enabling multilevel symmetries, i.e., symmetries within symmetries. Moreover, Lasso features represent distances to hyperplanes that are reflected across training points. These reflection hyperplanes are spanned by training data and are orthogonal to optimal weight vectors. Numerical experiments support theory and demonstrate theoretically predicted features when training networks using embeddings generated by Large Language Models.

==> 4layers_2neurons_extra.tex <==
%the 4 layers was done incorrectly. We used ReLU and made the mistake that weights that were supposed to be the same were actually independent. This is why we ignore this. There may be usome useful material thinking about 2 neurons whose weights sum to 1, to move away from the symmeterization restriction.
\section{4 layers with $d$ dimensional input}
\section{Remove}
In particular, we consider the $4$-layer 
%or absolute value
network with ReLU activation where $m_l = 1$ for all $l \in [L]$:
%There is one neuron in each hidden layer (ie, the layers preceded and followed by activations). 

\begin{equation}\label{eq:4lyrReLUdeepnarrow}
    \nn\left(\mathbf{x}\right) =  \sum_{i=1}^{m_4}  \left(  \left(  \left(\mathbf{x} \Wul{i}{1} + \sbul{i}{1} \right)_+ \sWul{i}{2} + \sbul{i}{2}  \right)_+ \sWul{i}{3} + \sbul{i}{3}  \right)_+ \sWul{i}{4} + \extbias.
\end{equation}
%
The internal weights and biases have dimensions $\Wul{i}{1} \in \mathbb{R}^d$, $\sWul{i}{l} \in \mathbb{R}$ for $l \in \{2,3,4\}$ and $ \sbul{i}{l} \in \mathbb{R}$ for $l \in [4]$.
In the training problem, we focus on $l_2$ norm loss and and $l_1$ norm regularization. This gives the training problem
 \begin{equation}\label{eq:trainingproblem_4lyrdeepnarrow}
    \min_{\params \in \Theta}  \frac{1}{2} \| \nn\left({\mathbf{X}}\right)  - \mathbf{y} \|^2_2 + \frac{\beta}{4} \left( \sum_{i=1}^{m_4} \left \|\Wul{i}{1} \right\|_{1}^4  + \sum_{l=2}^4 \left |\sWul{i}{l} \right |^4  \right)
\end{equation}
where $\nn$ is as defined in \eqref{eq:4lyrReLUdeepnarrow}.

For $\mathbf{j} = (j_1 ,  \cdots, j_{d-1}) \in [N]^{d-1}$ and $j_d \in [N]$  let $\vol_{i,\mathbf{j}} = \frac{\text{Vol} \left( \Delta_{j_1}, \cdots, \Delta_{j_{d-1}}, {\Delta}_{j_i} \right)_+}{ \left\| \Delta_{j_1} \times \cdots \times \Delta_{j_{d-1}} \right \|_1} $, where given $\mathbf{j}$, we define $\Delta_{i} = \mathbf{x}_i - \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \in \mathbb{R}^{1 \times d}$. We interpret $\Delta_{i}$ as distance vectors between training samples and their reflections. We interpret $\vol_{i,\mathbf{j}}$ as the signed, normalized volume of $d$ training samples.

%$\mathbf{v}^{(\mathbf{j})} = \Delta_{j_1} \times  \cdots \times \Delta_{j_{d-1}} \in \mathbb{R}^{d-1}, a = \| \mathbf{v}^{(\mathbf{j)}}\|_1$  $\vol_{i,\mathbf{j}} = \frac{1}{\| \times_{j=1}^{d-1} \Delta_j \|_1}\Delta_{j_1} \times  \cdots \times \Delta_{j_{d-1}} {\Delta}_{j_d}  = \frac{1}{\| \times_{j=1}^{d-1} \Delta_j \|_1}\text{Vol} \left( \Delta_{j_1}, \cdots, \Delta_{j_{d-1}}, {\Delta}_{j_d} \right)  $. %FIX x_j to x_j - other points, or canonical basis vectors. 

\begin{informalTheorem}{Theorem 1}
    The training problem \eqref{eq:trainingproblem_4lyrdeepnarrow} for a $4$-layer ReLU network is equivalent to the convex \lasso{} problem
    \begin{equation*}
\min_{\mathbf{z}, \xi}  \frac{1}{2} \| \Amat{} \mathbf{z} + \extbias \mathbf{1} - \mathbf{y} \|^2_2 + \beta \|\mathbf{z}\|_1,
	%\min_{\mathbf{z}} \mathcal{L}_{\mathbf{y}} (\mathbf{A}\mathbf{z} + \xi \mathbf{1}) + \frac{\beta}{2} \|\mathbf{z}\|_1,
\end{equation*}
%
where $\mathbf{A}$ is a dictionary matrix with columns of length $N$ whose $n^{\text{th}}$ element is 

\begin{equation*}
    \begin{aligned}
        f_n &= \left( \pm \left(  \left( \pm  \left(  \vol_{n,\mathbf{j}}   {-}  \vol_{j_2, \mathbf{j}} \right) \right)_+   {-} \left(  \pm \left(  \vol_{j_3, \mathbf{j}}  {-} \vol_{j_2, \mathbf{j}} \right) \right)_+ \right)  \right)_+
    \end{aligned}
\end{equation*} %FIX put sigma -> relu


\end{informalTheorem}
The rescaled problem when $l_1$ regularization is used in the training problem is 
 \begin{equation*}
    \min_{\params \in \Theta:\left\| \Wul{i}{l}\right\| = 1, l \in [L-1]} \lossfunc\left(\nn \left(\mathbf{X} \right) \right) + \beta \sum_{i=1}^{L} |\sWul{i}{L}|. 
\end{equation*}

%%%%%%%%%
Consider the $4$-layer deep narrow ReLU 
%or absolute value
network with training samples of dimension $d \geq 1$.
%There is one neuron in each hidden layer (ie, the layers preceded and followed by activations). 
In other words, the network is 

\begin{equation*}
    \nn{4}{\mathbf{x}} = \xi + \sum_{i=1}^{m_4} \alpha_i \sigma \left( \sigma \left( \sigma \left(\mathbf{x} \Wul{i}{1} + b^{(i,1)} \right) w^{(i,2)} + b^{(i,2)}  \right) w^{(i,3)} + b^{(i,3)}  \right),
\end{equation*}
%
with parameters $\Wul{i}{1} \in \mathbb{R}^d$, $w^{(i,l)} \in \mathbb{R}$  and $b^{(i,l)}, \alpha_i, \xi \in \mathbb{R}$ for $l \geq 1$.
%
Consider the training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro} but where the weight regularization is with $1$-norm, ie 

\begin{equation*}
    \min_{\params \in \Theta}  \frac{1}{2} \| \nn{L}{\mathbf{X}}  - \mathbf{y} \|^2_2 + \frac{\beta}{L} \left(\sum_{i=1}^{m_4}|\alpha_i|_1^L + \|\Wul{i}{1}\|_1^L + |w^{(i,2)} |^L  + |w^{(i,3)} |^L \right). 
\end{equation*}

%As before, bias parameters are unregularized.
By a similar argument as Lemma 27 in \citep{pilanci2023complexity}  and \cref{lemma:rescale}, %Lemma 8 in the 1D NN paper
the training problem can be rescaled to \cref{eq:noncvxtrain_genLlyrLLnorm_rescale}
%Equation (20) in the 1D NN paper,
but with $L$ changed to $1$ in the norm constraint $\|\Wul{i}{l}\|_{L}$. Its dual is \cref{gen_parallel_dual}.
%Equation (27) in the 1D NN paper. 
Note that for $\mathbf{w} \in \mathbb{R}^d$ and $\mathbf{a}, \mathbf{b} \in \mathbb{R}^{1 \times d}$, the "reflections" are $\reflect{\mathbf{a}}{\mathbf{b}} = 2\mathbf{b}-\mathbf{a} \in \mathbb{R}^{1 \times d}$ and $\reflect{\mathbf{aw}}{\mathbf{bw}} = 2\mathbf{bw}-\mathbf{aw}=(2\mathbf{b}-\mathbf{a})\mathbf{w}=\reflect{\mathbf{a}}{\mathbf{b}}\mathbf{w} \in \mathbb{R}$. The only difference from before is $\mathbf{W}^{(1)}$ and $\mathbf{x}_n$ are of length $d$ instead of being scalars. However, $\mathbf{x}_n \mathbf{W}^{(1)} \in \mathbb{R}$. Therefore \cref{lemma:max_constr_Llyrl}
% Lemma 10 in the 1D NN paper 
still holds with the same proof. By redefining the domains $s_1 \in \mathbb{R}^d$ instead of $s_1 \in \{-1,1\}$ and $\mathcal{\Tilde{M}}^{(1)} = \mathcal{M}^{(1)} = \mathbb{R}^{d} \times \{-1,1,\}^{L-2}$ instead of $ \{-1,1\}^{L}$ in \cref{def:tempreludicfunc} and \cref{def:dicindexset},
%Definition (10) in the 1D NN paper, 
\cref{lemma:L234constr_recursive}
% Lemma 11 in the 1D NN paper
holds. Now plug in optimal candidates for $b^{(1)}$ in the last equation in the proof of \cref{lemma:max_constr_Llyrl}. Let $\mathbf{j}=(j_1,j_2,j_3)$. The maximization constraint in the dual is 

\begin{equation*}
     \max_{\mathbf{j}, \mathbf{w}^{(i)}, \mathbf{a}\in \tilde{\params} }  \left | \sum_{n=1}^N \lambda_n f_n \right| \leq \beta,
\end{equation*}
where 
\begin{equation}\label{eq:fn}
    \begin{aligned}
        f_n &=  \sigma \left(  \left( \sigma \left(   \left( \sigma \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right)\mathbf{w}^{(1)} \right)  {-} \sigma \left(\left( {\mathbf{x}_{j_2}} {-} \mathbf{a} \right)\mathbf{w}^{(1)}  \right) \right) w^{(2)} \right) \right. \right. \\
     &   \qquad  {-}\sigma \left(  \left( \sigma \left(\left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right) \mathbf{w}^{(1)} \right)  {-} \sigma \left( \left( {\mathbf{x}_{j_2} } {-} \mathbf{a} \right)\mathbf{w}^{(1)} \right)  w^{(2)}\right) \right) \Big) w^{(3)} \Big)
    \end{aligned}
\end{equation}
%
%\begin{equation*}
%\begin{aligned}
%     \max_{\mathbf{j}, \mathbf{w}^{(i)}, a\in \tilde{\params} } & \Bigg | \sum_{n=1}^N \lambda_n \sigma \left(  \left( \sigma \left(   \left( \sigma \left( \left( \mathbf{x}_n {-} {a} \right)\mathbf{w}^{(1)} \right)  {-} \sigma \left(\left( {\mathbf{x}_{j_2}} {-} a \right)\mathbf{w}^{(1)}  \right) \right) w^{(2)} \right) \right. \right. \\
%     &  \qquad \qquad  {-}\sigma \left(  \left( \sigma \left(\left( {\mathbf{x}_{j_3}} {-} a \right) \mathbf{w}^{(1)} \right)  {-} \sigma \left( \left( {\mathbf{x}_{j_2} } {-} a \right)\mathbf{w}^{(1)} \right)  w^{(2)}\right) \right) \Big) w^{(3)} \Big) \Bigg | \leq \beta. 
%\end{aligned}
%\end{equation*}
%
and $\tilde{\params} = \left \{\mathbf{j}, \mathbf{w}, \mathbf{a}: j_1, j_2, j_3 \in [N], \mathbf{a} \in \left \{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right \}, w^{(3)} = \pm 1, w^{(2)} = \pm 1, \|\mathbf{w}^{(1)}\|_1=1 \right\}$. Note that $\mathbf{a}$ depends on $\mathbf{j}$.
Now, we make the constraints finite and the objective linear in $\mathbf{w}^{(1)}$ by optimizing $\mathbf{w}^{(1)}$ over polytopes defined by hyperplane arrangements. Denote $\mathbf{1}\{z\}$ as the threshold function outputting $1$ if $z \geq 0$ and $0$ otherwise, and extend it componentwise for vector inputs.
Define the following sets of  hyperplane arrangement patterns. 

%For  $j \in [N]$,
%\begin{equation*}
%   \mathcal{D}_j = \left \{ \text{Diag} \left( \mathbf{1} \left\{ \left(\mathbf{X}- \mathbf{1}\mathbf{x}_j \right) \mathbf{w} \right\} \right): \mathbf{w} \in \mathbb{R}^d \right\} 
%\end{equation*}
%and for $j_1, j_2 \in [N]$, 
%\begin{equation*}
%    \mathcal{D}^{R}_{(j_1,j_2)} = \left\{ \text{Diag} \left(
%\mathbf{1}\left\{ \left(\mathbf{X}- \mathbf{1}\reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}}\right) \mathbf{w}  \right \} \right): \mathbf{w} \in \mathbb{R}^d \right \}.
%\end{equation*}

For $\mathbf{j},a \in \tilde{\theta}$, let $\mathcal{D}_{\mathbf{j},\mathbf{a}} = \left \{ \text{Diag} \left( \mathbf{1} \left\{ \left(\mathbf{X}- \mathbf{1a} \right) \mathbf{w} \right\} \right): \mathbf{w} \in \mathbb{R}^d \right\} $. Enumerate $\left \{D_{\mathbf{j},\mathbf{a},1}, \cdots D_{\mathbf{j},\mathbf{a}, P} \right \} = \mathcal{D}_{\mathbf{j},\mathbf{a}}$. For $p \in [P]$, let $\mathcal{C}_{\mathbf{j},\mathbf{a},p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D_{\mathbf{j},\mathbf{a},p} -I\right) \left( \mathbf{X}-\mathbf{1}\mathbf{a} \right) \mathbf{w} \geq 0  \right \}$. 
Then, we have $\sigma \left(\left(\mathbf{X} - \mathbf{1}\mathbf{a} \right) \mathbf{w}^{(1)}  \right) = D_{\mathbf{j},\mathbf{a},p} \left(\mathbf{X}-\mathbf{1}\mathbf{a}\right) \mathbf{w}^{(1)} $  iff $\mathbf{w}^{(1)} \in \mathcal{C}_{\mathbf{j},\mathbf{a},p} $. 

As a special case when $\mathbf{a}$ is a data sample, for $j \in [N]$ and $w \in \mathbb{R}^d$, let $\mathcal{D}_{j} $ be $ \mathcal{D}_{\mathbf{j},\mathbf{a}}$ where $\mathbf{a}=\mathbf{x}_j$. For $j \in [N] $, enumerate $\left \{D_{j,1}, \cdots, D_{j,P_j} \right \} = \mathcal{D}_{j}$. As similar to above, let $\mathcal{C}_{j,p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D_{j,p} -I\right)\left( \mathbf{X}-\mathbf{1}\mathbf{x}_j \right) \mathbf{w} \geq 0  \right \}$.  
%
%Let $\left \{D_{j,1}, \cdots D_{j,P_j} \right \} = \mathcal{D}_j$. For $j \in [N]$, $p \in [P_j]$, let $\mathcal{C}_{j,p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D_{j,p} -I\right) \mathbf{X} \mathbf{w} \geq 0  \right \}$. Then, for $j \in [N]$, $p \in [P_j]$, we have $\sigma \left(\left(\mathbf{X} - \mathbf{1}\mathbf{x}_j \right) \mathbf{w}^{(1)}  \right) = D_{j,p} \left(\mathbf{X}-\mathbf{1}\mathbf{x}_j \right) \mathbf{w}^{(1)} $  iff $\mathbf{w}^{(1)} \in \mathcal{C}_{j,p} $.
%
%Similarly let $\left \{ D^R_{(j_1,j_2),1}, \cdots D^R_{(j_1,j_2),P_{(j_1,j_2)}} \right\} = \mathcal{D}^R_{(j_1, j_2)}$. For $j_1, j_2 \in [N]$, $p \in [P_{(j_1, j_2)}]$, let $\mathcal{C}^R_{(j_1, j_2),p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D^R_{(j_1,j_2),p} -I\right) \mathbf{X} \mathbf{w} \geq 0  \right \}$. Then, for $j_1, j_2 \in [N]$, $p \in [P_{(j_1, j_2)}]$, we have $\sigma \left(\left(\mathbf{X} - \mathbf{1}\reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right) \mathbf{w}^{(1)}  \right) = D^R_{(j_1, j_2),p} \left(\mathbf{X}-\mathbf{1}\reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}}\right) \mathbf{w}^{(1)} $  iff $\mathbf{w}^{(1)} \in \mathcal{C}^R_{(j_1, j_2),p} $.
%
%Therefore, for fixed $\mathbf{j}$, if $a =x_{j_1}$ then for $\mathbf{w}^{(1)} \in \mathcal{C}_{j_1,p} $,
%
%\begin{equation*}
%    \begin{aligned}
%        f_n &=  \sigma \left(  \left( \sigma \left(   \left( \left( \mathbf{x}_n {-} {a} \right)\mathbf{w}^{(1)}{\left(D_{j_1,p}\right)}_n   {-} \left( {\mathbf{x}_{j_2}} {-} a \right)\mathbf{w}^{(1)}  {\left(D_{j_1,p}\right)}_{j_2} \right) w^{(2)} \right) \right. \right. \\
%     &   \qquad  {-}\sigma \left(  \left( \left( {\mathbf{x}_{j_3}} {-} a \right) \mathbf{w}^{(1)} {\left(D_{j_1,p}\right)}_{j_3}  {-}  \left( {\mathbf{x}_{j_2} } {-} a \right)\mathbf{w}^{(1)} {\left(D_{j_1,p}\right)}_{j_2} \right) w^{(2)}\right) \Big) w^{(3)} \Big) \\
%     & = \sigma \left(  \left( \sigma \left(   \left(  \mathbf{x}_n {-} {a}   {-} \left( {\mathbf{x}_{j_2}} {-} a \right) {\left(D_{j_1,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{j_1,p}\right)}_n \right) \right. \right. \\
%     &    \qquad {-}\sigma \left(  \left(  {\mathbf{x}_{j_3}} {-} a     {-}  \left( {\mathbf{x}_{j_2} } {-} a \right){\left(D_{j_1,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{j_1,p}\right)}_{j_3}\right) \Big) w^{(3)} \Big) \\
%    \end{aligned}
%\end{equation*}
%
%and similarly with $D^R_{j_1, j_2, p}$ instead of $D_{j_1, p}$ if $a = \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}}$.
%
%Let $D_{\mathbf{j},a,p}$ be $D_{j_1,p}$

For $w \in \{-1,1\}$, and $d \in \{0,1\}$, let $\Bar{d}=1-d$ and $d^{w}$ be $d$ if $w=1$ and $1-d$ if $w=-1$.

Fix $\mathbf{j},\mathbf{w},\mathbf{a} \in \Tilde{\theta}$. Fix $p \in [P], p_{j_2} \in [P_{j_2}], p_{j_3} \in [P_{j_3}]$. For $i \in [N]$, let $d_{\mathbf{a},i} = \left(D_{\mathbf{j},\mathbf{a},p}\right)_{i,i} \in \{0,1\}$. For $j,i\in [N]$, let $d_{j, i} = \left(D_{j,p_j}\right)_{i,i} \in \{0,1\}$. 
 When $\mathbf{w}^{(1)} \in \mathcal{C}_{\mathbf{j},\mathbf{a},p} \cap \mathcal{C}_{j_2, p_{j_2}} \cap \mathcal{C}_{j_3, p_{j_3}}$, we have

\begin{equation*}
    \begin{aligned}
    f_n &=  \sigma \left(  \left( \sigma \left(   \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right)\mathbf{w}^{(1)}d_{\mathbf{a,n}}   {-} \left( {\mathbf{x}_{j_2}} {-} \mathbf{a} \right)\mathbf{w}^{(1)} d_{\mathbf{a},j_2}  \right) w^{(2)} \right) \right. \right. \\
     &   \qquad  {-}\sigma \left(  \left( \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right) \mathbf{w}^{(1)} d_{\mathbf{a},j_3} {-}  \left( {\mathbf{x}_{j_2} } {-} \mathbf{a} \right)\mathbf{w}^{(1)} d_{\mathbf{a},j_2} \right) w^{(2)}\right) \Big) w^{(3)} \Big) \\
     %
     %& = \sigma \left(  \left( \sigma \left(   \left(  \mathbf{x}_n {-} {a}   {-} \left( {\mathbf{x}_{j_2}} {-} a \right) {\left(D_{\mathbf{j},a,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{\mathbf{j},a,p}\right)}_n \right) \right. \right. \\
     %&    \qquad {-}\sigma \left(  \left(  {\mathbf{x}_{j_3}} {-} a     {-}  \left( {\mathbf{x}_{j_2} } {-} a \right){\left(D_{\mathbf{j},a,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{\mathbf{j},a,p}\right)}_{j_3}\right) \Big) w^{(3)} \Big) \\
     %
     &= \sigma \left(  \left( \sigma \left(   \left(  \left( \mathbf{x}_n {-} {\mathbf{a}} \right)d_{\mathbf{a},n} \Bar{d}_{\mathbf{a},j_2}+ (\mathbf{x}_n {-} \mathbf{x}_{j_2})d_{\mathbf{a},n} d_{\mathbf{a},j_2} - \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{a},j_2} \right) \mathbf{w}^{(1)} w^{(2)}  \right)  \right. \right. \\
     &    \qquad {-}\sigma \left(  \left(  \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right)d_{\mathbf{a},j_3}\Bar{d}_{\mathbf{a},j_2}  + \left( \mathbf{x}_{j_3} {-}\mathbf{x}_{j_2}\right)d_{\mathbf{a},j_3}d_{\mathbf{a},j_2} - \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{a,j_3}d_{\mathbf{a},j_2}  \right) \mathbf{w}^{(1)} w^{(2)} \right) \Big) w^{(3)} \Big) \\
     %
      %&= \sigma \left(  \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right) d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_2} d^{w^{(2)}}_{\mathbf{a},n}  + (\mathbf{x}_n {-} \mathbf{x}_{j_2})d_{\mathbf{a},n}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,n} + \left( \mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{a},j_2} d^{-w^{(2)}}_{\mathbf{a},j_2} 
     %   \right. \right.  \\
     %&   \qquad {-}   \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right)d_{\mathbf{a},j_3}\Bar{d}_{\mathbf{a},j_2}d^{w^{(2)}}_{\mathbf{a},j_3}  - \left( \mathbf{x}_{j_3} {-}\mathbf{x}_{j_2}\right)d_{\mathbf{a},j_3}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,j_3} - \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right)  \Bar{d}_{a,j_3} d_{\mathbf{a},j_2} d^{-w^{(2)}}_{\mathbf{a},j_2}   \Big) \mathbf{w}^{(1)} w^{(3)} \Big) \\
     %
    &= \sigma \left(  \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right) d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}1\right\}
    + (\mathbf{x}_n {-} \mathbf{x}_{j_2})d_{\mathbf{a},n}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,n} 
    + \left( \mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}-1\right\}
        \right. \right.  \\
     &   \qquad {-}   \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right)d_{\mathbf{a},j_3}\Bar{d}_{\mathbf{a},j_2}\mathbf{1}\left\{w^{(2)}{=}1\right\} 
     - \left( \mathbf{x}_{j_3} {-}\mathbf{x}_{j_2}\right)d_{\mathbf{a},j_3}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,j_3} -
     \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right)  \Bar{d}_{\mathbf{a},j_3} d_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}{-}1\right\}   \Big) \mathbf{w}^{(1)} w^{(3)} \Big) \\ 
     %
     & \scalemath{0.8}{
     {=} \left( \left(\left(\mathbf{x}_n {-} \mathbf{a}\right)d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_3}\mathbf{1}\left \{w^{(3)}{=}1 \right\} 
     {+} \left(\mathbf{x}_n {-} \mathbf{x}_{j_3}\right)d_{\mathbf{a},n}d_{\mathbf{a},j_3}d^{w^{(3)}}_{j_3,n} {-} \left(\mathbf{x}_{j_3} {-} \mathbf{a}\right)\Bar{d}_{\mathbf{a},n}d_{\mathbf{a},j_3}\mathbf{1}\left\{w^{(3)}{=}{-}1\right\} \right)\Bar{d}_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}1\right\} \right.
     }\\
     & \scalemath{0.8}{ 
     {+} \left(\left(\mathbf{x}_n {-} \mathbf{x}_{j_2} \right) d_{\mathbf{a},n} \Bar{d}_{\mathbf{a},j_3}d_{j_2, n} \mathbf{1}\left \{ w^{(3)}{=}1\right\}{+} \left(\mathbf{x}_n {-}\mathbf{x}_{j_3} \right) d_{\mathbf{a},n} d_{\mathbf{a},j_3}d_{j_2,n}d_{j_2,j_3}d_{j_3,n}^{w^{(3)}} {+} \left(\mathbf{x}_{j_3} {-} \mathbf{x}_{j_2} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{\mathbf{a}},j_3}d_{j_2,j_3} \mathbf{1}\left\{ w^{(3)}{=}{-}1\right\}\right) d_{\mathbf{a},j_2} \mathbf{1} \left\{ w^{(2)}{=}1\right\}
     } \\
     & {+} \left(\mathbf{x}_{j_2}{-}\mathbf{a} \right)\left(\bar{d}_{\mathbf{a},n}d_{\mathbf{a},j_3} \mathbf{1}\left\{ w^{(3)}{=}1\right\}{+} d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_3}  \mathbf{1}\left\{ w^{(3)}{=-}1\right\}\right)d_{\mathbf{a},j_2} \mathbf{1}\left \{w^{(2)}{=}{-}1 \right \} \Big) \mathbf{w}^{(1)} 
    \end{aligned}
\end{equation*}
%
which is linear in $\mathbf{w}^{(1)}$.
%and in every case, the argument of $\sigma(\cdot)$ will be of the form $(\mathbf{x}_{j}-\mathbf{a})\mathbf{w}^{(1)}\mathbf{w}^{(3)}$ where $\mathbf{a}$ is a data point or a reflection of data points, so the $\sigma$ can be removed by inserting hyperplane arrangement matrices.
Let $\mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}} = \mathcal{C}_{\mathbf{j},\mathbf{a},p} \cap \mathcal{C}_{j_2, p_{j_2}} \cap \mathcal{C}_{j_3, p_{j_3}} \cap \{\mathbf{w} \in \mathbb{R}^{d}: \|\mathbf{w}^{(1)}\|_1=1 \}$.
Therefore the maximization constraint in the dual is

\begin{equation*}
    \max_{j_1, j_2, j_3 \in [N] } 
    \max_{\mathbf{a} \in \left\{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}} 
    \max_{w^{(2)}, w^{(3)} \in \{-1,1\}} \max_{p \in [P], p_{j_2} \in [P_{j_2}], p_{j_3} \in [P_{j_3}]}
    \max_{\mathbf{w}^{(1)} \in \mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}} }  \left | \sum_{n=1}^N \lambda_n f_n \right| \leq \beta.
\end{equation*}
%
Since a linear function $\pm \sum_{n=1}^N \lambda_n f_n$ is being maximized over a polytope $\mathcal{E}_{\mathbf{j},\mathbf{a},\mathbf{p}}$, it suffices to maximize 
$f_n$ over the finite set of extremal points of $\mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}}$. By Lemma 19 in \citep{pilanci2023complexity}, the set of extremal points of $\mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}}$ are

\begin{equation*}
\mathcal{E}_{\mathbf{j},\mathbf{a},\mathbf{p}} = \left \{w \in  \mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}}: \exists S \subset [N], |S| = d-1, \text{ s.t. } \mathbf{M}_s w =\mathbf{0}, \text{ rank}(\mathbf{M}_s)=d-1 \right \},
\end{equation*}
where 

\begin{equation*}
\mathbf{M} = 
    \begin{pmatrix}
        \mathbf{X} - \mathbf{1}\mathbf{a} \\
         I
    \end{pmatrix}.
\end{equation*}
%
Note that $\mathbf{M}$ depends on $\mathbf{j}$ and $\mathbf{a}$. Writing $f_n$ in its equivalent form \eqref{eq:fn}, the objective and $\mathcal{E}_{\mathbf{j},\mathbf{a},\mathbf{p}}$ depend on $\mathbf{j}$ and $\mathbf{a}$ but not on $\mathbf{p}$. For each $\mathbf{j},\mathbf{a}$, the union of the regions $\mathcal{C}_{\mathbf{j},\mathbf{a},p} \cap \mathcal{C}_{j_2, p_{j_2}} \cap \mathcal{C}_{j_3, p_{j_3}} $ over $\mathbf{p}$ cover all of $\mathbb{R}^N$. So the maximization constraint is equivalent to  

\begin{equation*}
    \max_{j_1, j_2, j_3 \in [N] } 
    \max_{\mathbf{a} \in \left\{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}} 
    \max_{w^{(2)}, w^{(3)} \in \{-1,1\}} 
    \max_{\mathbf{w}^{(1)} \in \mathcal{E}_{\mathbf{j},\mathbf{a}} }  \left | \sum_{n=1}^N \lambda_n f_n \right| \leq \beta,
\end{equation*}
%
where
%
\begin{equation*}
\mathcal{E}_{\mathbf{j},\mathbf{a}} = \left \{w \in \mathbb{R}^d: \exists S \subset [N], |S| = d-1, \text{ s.t. } \mathbf{M}_s w =\mathbf{0}, \text{ rank}(\mathbf{M}_s)=d-1 \right \}.
\end{equation*}

Consider the \lasso{} problem

\begin{equation*}
\min_{\mathbf{z}, \xi}  \frac{1}{2} \| \Amat{} \mathbf{z} + \xi \mathbf{1} - \mathbf{y} \|^2_2 + \beta \|\mathbf{z}\|_1,
	%\min_{\mathbf{z}} \mathcal{L}_{\mathbf{y}} (\mathbf{A}\mathbf{z} + \xi \mathbf{1}) + \frac{\beta}{2} \|\mathbf{z}\|_1,
\end{equation*}
%
where $\mathbf{A}$ is a dictionary matrix with columns of length $N$ whose $n^{\text{th}}$ element is $f_n$ as defined in \eqref{eq:fn}, for each $j_1,j_2,j_3 \in [N], \mathbf{a} \in \left \{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}$, $\mathbf{w}^{(1)} \in \mathcal{E}_{\mathbf{j},\mathbf{a}}$, and $w^{(2)}, w^{(3)} \in \{-1,1\}$.
%
As the bidual of the training problem, the \lasso{} problem is a lower bound for the training problem. We now describe a reconstruction from a \lasso{} solution $\mathbf{z}^*, \xi^*$ to a neural net that is optimal in the training problem, as similar to \cref{def:reconstructfunc}. We assume that $m_4 \geq \|\mathbf{z}^*\|_0$.
%For each $j_1,j_2,j_3 \in [N], \mathbf{a} \in \left \{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}$, $\mathbf{w}^{(1)} \in \mathcal{E}_{\mathbf{j},\mathbf{a}}$, and $w^{(2)}, w^{(3)} \in \{-1,1\}$, the corresponding \lasso{} feature is a column in $\mathbb{R}^N$ with $n^{\text{th}}$ element \eqref{eq:fn}.
For each $i^{\text{th}}$ selected feature of the \lasso{} problem and corresponding $\mathbf{w}^{(1)}, w^{(2)}, w^{(3)}$ and feature coefficient $z^*_i$, let $\mathbf{a}_1 = \mathbf{a} \in \mathbb{R}^{1 \times N}$, $a_2 = \left(\left(\mathbf{x}_{j_2} -\mathbf{a}_1 \right)\mathbf{w}^{(1)} \right)_+ \in \mathbb{R}$, $a_3 = \left(  \left(\left(  \left( \mathbf{x}_{j_3} - \mathbf{a}_1 \right)\mathbf{w}^{(1)} \right)_+ - a_2\right)w^{(2)} \right)_+ \in \mathbb{R}$.
  Let  $ \boldsymbol{\alpha} = \mathbf{z}^*$ and $\xi=\xi^*$. 
  Let $\Wul{i}{1} = \mathbf{w}^{(1)}, w^{(i,l)} = w^{(l)} 
  %\in \{-1,1\}$
  $, $\bul{i}{1} = - \mathbf{a}_1 \mathbf{w}^{(1)}, b^{(i,l)} = - a_l w^{(l)}
  %\in \mathbb{R}
  $.
  Finally, let $\gamma_i = |\alpha_i|^{\frac{1}{4}}$ and apply the transformation $q \to \gamma_i \frac{q}{\|q\|_1}$ for $q \in \left\{\alpha_i, \Wul{i}{1}, w^{(i,2)}, w^{(i,3)}  \right\}$, and $b^{(i,l)} \to b^{(i,l)} \left(\gamma_i\right)^l $. 
Let these be weights for that $i^{\text{th}}$ parallel unit. This reconstructs a neural net that achieves the same objective, showing that the \lasso{} problem is equivalent to the training problem. %: 
%$a^{(1)} = \mathbf{a}, b^{(i,2)} = -\left(\left(\mathbf{x}_{j_2} - b^{(i,1)} \right)\mathbf{w}^{(1)} \right)_+ w^{(2)}$, $b^{(i,3)} = -\left(  \left(\left(  \left( \mathbf{x}_{j_3} - a^{(i)}_1 \right)\mathbf{w}^{(1)} \right)_+ - a^{(i)}_2\right)s_{2} \right)_+ w^{(3)}$ for the third layer.

While $w^{(2)}, w^{(3)} \in \{-1,1\}$ (up to rescaling the network), the values of $\mathbf{w}^{(1)}$ are the elements of $\mathcal{E}_{\mathbf{j},\mathbf{a}}$. By the orthogonality characterization,

\begin{equation*}
   \mathcal{E}_{\mathbf{j},\mathbf{a}} = \left\{ \frac{\times_{\tilde{\mathbf{x}}_n \in \Tilde{\mathbf{X}}} \Tilde{\mathbf{x}}_n }{\|\times_{\Tilde{\mathbf{x}}_n \in \Tilde{\mathbf{X}}} \Tilde{\mathbf{x}}_n \|_1} \right\},
\end{equation*}
%
where $\Tilde{\mathbf{X}}$ is a set of $d-1$ linearly independent vectors in $\{\mathbf{x}_1-\mathbf{a}, \cdots, \mathbf{x}_N-\mathbf{a}, \mathbf{e}_1, \cdots, \mathbf{e}_d\}$. For each first layer weight $\mathbf{w}^{(1)}$, there is a training sample or its reflection for which $\mathbf{w}^{(1)}$ is orthogonal to at least $d-1$ other training samples shifted by it.

\section{2 layers with $>1$ neuron}

Suppose $\mathbf{w}^{(1)} \in \mathbb{R}^{d \times M}, \mathbf{b}^{(1)} \in \mathbb{R}^{1 \times M}, \mathbf{w}^{(2)} \in \mathbb{R}^{M \times 1}$ and $b^{(2)}, w^{(3)}, b^{(3)}  \in \mathbb{R}$. Then optimizing the maximization constraint in the dual over $b^{(3)}, b^{(2)}$ gives

\begin{equation*}
    \begin{aligned}
        f_n &=  \sigma \left(  \left( \sigma \left(   \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)} {+} \mathbf{b}^{(1)}\right)  {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}  {+}  \mathbf{b}^{(1)}  \right) \right) \mathbf{w}^{(2)} \right) \right. \right. \\
     &   \qquad  {-}\sigma \left(  \left( \sigma \left({\mathbf{x}_{j_3}}\mathbf{w}^{(1)}  {+} \mathbf{b}^{(1)}  \right)  {-} \sigma \left( {\mathbf{x}_{j_2} } \mathbf{w}^{(1)}{+} \mathbf{b}^{(1)}\right) \right)  \mathbf{w}^{(2)} \right) \Big) w^{(3)} \Big) \\
     %
     &=  \sigma \left(  \left( \sigma \left(  \sum_{m=1}^M  \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,m} {+} b^{(1)}_m  \right) {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,m}  {+}  b^{(1)}_m  \right) \right) w^{(2)}_m \right) \right. \right. \\
     &   \qquad  {-}\sigma \left( \sum_{m=1}^M \left( \sigma \left({\mathbf{x}_{j_3}}\mathbf{w}^{(1)}_{:,m}  {+} b^{(1)}_m  \right)  {-} \sigma \left( {\mathbf{x}_{j_2} } \mathbf{w}^{(1)}_{:,m}{+} b^{(1)}_m\right) \right) w_m^{(2)} \right) \Bigg) w^{(3)} \Bigg)
    \end{aligned}
\end{equation*}

Suppose there are $3$ layers and $2$ neurons in each layer. Let 
\begin{equation*}
    c_m = \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,m} 
     {+} b^{(1)}_m \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,m}  
     {+}  b^{(1)}_m \right) \right) w^{(2)}_m \in \mathbb{R}.
\end{equation*}
%
     Then

\begin{equation*}
    \begin{aligned}
     f_n &=  \sigma \left(c_1 + c_2 \right).
    \end{aligned}
\end{equation*}
%
For fixed $\mathbf{w}^{(1)},\mathbf{w}^{(2)}_2$, note that $c_2$ does not depend on $b^{(1)}$ and $f_n$ is a capped ramp vertically shifted by $-c_2$. Then the \kink{}s of the piecewise linear function $\sum_{n=1}^N \lambda_n f_n$ as a function of $b^{(1)}_1 \in \mathbb{R}$ are at $b^{(1)}_1 \in \left\{-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1},-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1}-c_2  : j_1 \in [N] \right\} $.

%Feature shapes below. Also get as linear as possible with w
\textbf{Case 1}: If $b^{(1)}_1 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1}$ then $c_1$ is fixed for fixed $\mathbf{w}^{(1)},w^{(2)}$ and does not depend on $b^{(2)}$ and the \kink{}s of $\sum_{n=1}^N \lambda_n f_n$ as a function of $b^{(1)}_2 $ are $b^{(1)}_2 \in \left\{-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2},-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}-c_1  : j_1 \in [N] \right\} $. If moreover $b^{(1)}_2 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}$ then 

\begin{equation*}
    f_n = \sigma \left(\sum_{m=1}^2 \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,m} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,m} \right)\right) w^{(2)}_m   \right).
\end{equation*}
%
%this is a vector equation in terms of $\mathbf{x}_n$. Hard to call it a ramp, more like a 2D ramp
which is like a vertically shifted capped ramp in $2D$ in terms of $\mathbf{x}_n$ with \kink{} lines at \\ $\mathbf{x} \in \left \{ \mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1},\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}, \sum_{m=1}^2 \sigma \left( \left({\mathbf{x}_{j_2}} 
{-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,m} \right) w^{(2)}_m  \right \}$. 
If on the other hand 
$b^{(1)}_2 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}-c_1$ then

\begin{equation*}
   \begin{aligned}
    f_n &= \sigma \left( \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1 \right. \\  
     & \qquad {+} \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,2} -  \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1\right) \right. \\
     & \qquad {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,2}
     {-} \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1 \right)\Big) w^{(2)}_2 \Big) \Big) \\
     %
    % &=\sigma \left( \left( \sigma \left( \left( \mathbf{x}_n 
     %{-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     %{-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     %{-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1 \right. \\  
     %& \qquad {+} \left( \sigma \left( \left( \mathbf{x}_n 
     %{-} \mathbf{x}_{j_1} \right) \left(\mathbf{w}^{(1)}_{:,2} {-} \mathbf{w}^{(1)}_{:,1}w^{(2)}_1 \right)   
     %{+} \sigma \left( \left({\mathbf{x}_{j_2}} 
     %{-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)w^{(2)}_1 \right) \right. \\
   \end{aligned}
\end{equation*}

\textbf{Case 2}: If $b^{(1)}_1 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1}-c_2$ then $c_1$ depends on $b^{(1)}_2$ and in terms of $b^{(1)}_2$, we have

\begin{equation*}
\begin{aligned}
    f_n &= \sigma \left( \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} -\left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,2} 
     {+} b^{(1)}_2 \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,2}  
     {+}  b^{(1)}_2 \right) \right) w^{(2)}_2 \right. \right. \right) \\ 
     &\qquad {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} {-} \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,2} 
     {+} b^{(1)}_2 \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,2}  
     {+}  b^{(1)}_2 \right) \right) w^{(2)}_2  \right) \Big) w^{(2)}_1   \\
     &\qquad {+} \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,2} 
     {+} b^{(1)}_2 \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,2}  
     {+}  b^{(1)}_2 \right) \right) w^{(2)}_2 \Big).
\end{aligned}
\end{equation*}
which has \kink{}s and hence optimal $b^{(1)}_2$ when $b^{(1)}_2 \in ...$. 


If there were $M=2$ neurons in the second layer, I think this can be simplified.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

